AutoTriggER: Label-Efficient and Robust Named Entity Recognition with Auxiliary Trigger Extraction

Deep neural models for named entity recognition (NER) have shown impressive results in overcoming label scarcity and generalizing to unseen entities by leveraging distant supervision and auxiliary information such as explanations. However, the costs of acquiring such additional information are generally prohibitive. In this paper, we present a novel two-stage framework (AutoTriggER) to improve NER performance by automatically generating and leveraging ``entity triggers'' which are human-readable cues in the text that help guide the model to make better decisions. Our framework leverages post-hoc explanation to generate rationales and strengthens a model's prior knowledge using an embedding interpolation technique. This approach allows models to exploit triggers to infer entity boundaries and types instead of solely memorizing the entity words themselves. Through experiments on three well-studied NER datasets, AutoTriggER shows strong label-efficiency, is capable of generalizing to unseen entities, and outperforms the RoBERTa-CRF baseline by nearly 0.5 F1 points on average.

==> sections/backup-bill-revisions.tex <==
\section{Introduction} 
Named Entity Recognition (NER) serves as a key building block in information extraction systems and has broad applications for many domains.
Recent advances in neural models for NER have yielded state-of-the-art performance when sufficient human annotations are available~\cite{Lample2016NeuralAF}.
However, these supervised learning methods are particularly challenging in specific domains, especially in technical domains such as biomedical, financial, legal reports, etc., where domain-expert annotations are expensive and slow to obtain.
This problem has been partially solved by various types of human-curated distant supervision such as entity dictionaries~\cite{autoner, yangner, Liu2019TowardsIN}, rules~\cite{safranchik:aaai20}, and labeling explanations~\cite{lin-etal-2020-triggerner, lee-etal-2020-lean}.
They show that asking humans to provide distant supervision is more cost-effective than collecting additional annotations.

\begin{figure}[t]
    \centering 
    \includegraphics[scale=0.5]{figures/overview.pdf}
    \caption{Existing distant supervised NER frameworks mostly rely on human provided additional supervision (e.g., labeling explanation). Unlike existing works, our framework automatically generates and leverage distant supervision to NER.}
    \label{fig:overview}
\end{figure}

In this paper, we focus on extracting distant supervision automatically and leveraging it to NER framework.
Here, distant supervision is an \textit{entity trigger}, an effective proxy of human explanation, which is defined as a group of words in a sentence that helps to explain why humans would recognize an entity in the sentence~\cite{lin-etal-2020-triggerner}.
For instance, we could infer that ``\textit{Sunnongdan}'' is likely to be a restaurant entity in the sentence ``\textit{Danny had a dinner at Sunnongdan last week, where the food is delicious.}''.
We could recognize this entity since the cue phrases ``\textit{had a dinner at}'' and ``\textit{where the food}'' both suggest there should be a restaurant entity between them.
We call such rationale phrases \textit{entity trigger (or. trigger)}.

Prior works on trigger-aware NER primarily use a limited number of crowd-soured triggers.
Although such triggers are of better quality, the crowd-sourcing procedure can be very expensive and time-consuming, as annotators are asked to provide both entity labels and their associated triggers in specifically designed annotation frameworks such as LEAN-LIFE~\cite{lee-etal-2020-lean}.
This largely limits the scale and domains of entity triggers. 
In addition, these trigger-aware NER models (e.g., Trigger Matching Networks~\cite{lin-etal-2020-triggerner}) are built on  conventional sequence tagging architectures, e.g., BLSTM-CRFs~\cite{Lample2016NeuralAF}.
Few works connect entity triggers with contextualized embeddings from pre-trained language models such as BERT~\cite{Devlin2019BERTPO}, which can be highly beneficial for low-resource languages.
In this paper, we propose a novel two-stage NER framework, named \autotrigger, that can \textit{automatically} generate and exploit entity triggers with  pre-trained language models towards better generalization.

The \textit{first} stage of our framework (Sec.~\ref{ssec:soc}) aims to \textit{automatically extract entity triggers} by saliency map technique based on input perturbations. 
Most saliency map techniques primarily focus on modeling the relative importance of each input token based on its 1) attention intensity~\cite{}, 2) gradients~\cite{} or 3) the changes of the output by excluding it from the input~\cite{}.
These methods can indeed produce useful explanations for some sentence classification tasks such as sentiment analysis, however, they are not well-aligned to our desired entity triggers --- a (potentially discontinuous) group of input tokens that often posses structural constraints to a target entity.
% \billquestion{can we have an example here?}
To address this challenge, we exploit the syntactic signals of sentences for properly assigning importance scores to a group of input tokens such that we can extract useful entity triggers without human efforts.
Specifically, 
for a given sentence and a target entity in it,
we first extract phrases from its \textit{constituency parsing tree}~\cite{} to form a collection of trigger candidates. 
Then, we score each trigger candidate by
testing its ability to predict the target entity in a variety of sampled contexts.
Here, we use the \textit{average score differences} between original inputs and trigger-free inputs as the metric.
The rationale here is the intuition that a better trigger should be robust and help recognize the target entity in many different context.
We find that such a \textit{sampling-and-occlusion}  method can automatically extracts triggers of high quality.
% computing the \textit{average score differences} between the input \textit{with} and \textit{without} the phrase in different context around the target candidate.
\billquestion{Add a concrete example? or reusing the one in the 2nd paragraph. }

The \textit{second} stage  (Sec.~\ref{ssec:tin})
focuses on how to use the extracted triggers for better performance and generalization of NER.
We propose \textit{Trigger Interpolation Network} (TIN), a novel architecture that effectively uses trigger-labeled NER data to train a model.
As a trigger is the most important non-entity words in an input sentence,
we want to strengthen such prior knowledge in a neural network model, instead of solely memorizing the entity words themselves.
Thus, we first mask the entity words and trigger words respectively, and then interpolate the embeddings of both entity-masked and trigger-masked sentences as the input to learn a mixed sentence representation as the input to standard sequence labeling.
Therefore, the TIN can effectively learn to exploit the triggers to infer entity boundary and type with the powerful contextualized embeddings from pre-trained language models such as BERT.
% We leverages both entity triggers and pre-trained language model (BERT~\cite{}) into the NER task.
% We propose a novel model architecture that interpolates an entity masked sentence and trigger masked sentence.
% The underlying intuition of our proposed model is as follows:
% 1) For entity masked sentence, can the entity trigger itself determine the masked entity label?
% 2) For entity trigger masked sentence, how does the entity label prediction change when the entity triggers are masked?
% By interpolating the embedding outputs of both sentences, we could effectively model the relationship between entity and entity trigger.

Extensive experimental results on various domains of NER dataset show that our framework consistently outperforms baseline methods.
~\textcolor{red}{TODO: Mention human in the loop}

==> sections/backup-liz-revisions.tex <==
\textbf{[[REVISED ABSTRACT LIZ)]]}

While deep neural models for named entity recognition (NER) have shown impressive results, these models often require human annotation that is expensive and time-consuming, especially for new or low-resource domains.
Some success has been shown replacing conventional human annotation with distant supervision or other meta-level information (e.g.\ explanations). However, the costs of generating this additional information can still be prohibitive, especially in domains where existing resources (e.g. databases to be used for distant supervision) may not exist.
In this paper, we present a novel two-stage framework (\textsc{AutoTriggER}) to improve NER performance by \textit{automatically} generating and leveraging ``triggers'' for named entity recognition. These triggers---essentially human-readable ``clues'' in text that can help guide the model to better decisions---are first identified automatically using a \textit{sampling and occlusion algorithm}. Next, we propose a \textit{trigger interpolation network} to leverage these triggers in a transformer-based NER model. By combining these stages, \textsc{AutoTriggER} is able to both create and leverage additional supervision by itself.
Through experiments on three well-studied NER datasets, we show that our automatically extracted triggers are well-matched to human triggers, and \textsc{AutoTriggER} improves performance over a standard BERT-CRF architecture by nearly 1.5 F1 points on average.


\textbf{[[REVISED INTRODUCTION LIZ]]}

Named Entity Recognition (NER) serves as a key building block in information extraction systems and has broad applications for many domains.
Recent advances in neural models for NER have yielded state-of-the-art performance when sufficient human annotations are available~\cite{Lample2016NeuralAF}.
However, these supervised learning methods are particularly challenging in specific domains, especially in technical domains such as biomedical, financial, legal reports, etc., where domain-expert annotations are expensive and slow to obtain.
This problem has been partially solved by various types of human-curated distant supervision such as entity dictionaries~\cite{autoner, yangner, Liu2019TowardsIN}, rules~\cite{safranchik:aaai20}, and labeling explanations~\cite{lin-etal-2020-triggerner, lee-etal-2020-lean}.
They show that asking humans to provide distant supervision is more cost-effective than collecting additional annotations.

\begin{figure}[t]
    \centering 
    \includegraphics[scale=0.5]{figures/overview.pdf}
    \caption{Existing distant supervised NER frameworks mostly rely on human provided additional supervision (e.g., labeling explanation). Unlike existing works, our framework automatically generates and leverage distant supervision to NER.}
    \label{fig:overview}
\end{figure}

In this paper, we focus on \textit{automatically} extracting distant supervision for NER, in the form of  \textit{entity triggers}. Entity triggers serve as an effective proxy of human explanation and are defined as a group of words in a sentence that helps to explain why humans would recognize an entity in the sentence~\cite{lin-etal-2020-triggerner}.
For instance, a human could infer that ``\textit{Sunnongdan}'' is likely to be a restaurant entity in the sentence ``\textit{Danny had a dinner at Sunnongdan last week, where the food is delicious.}''---despite never having seen the word \textit{Sunnongdan} before. 
This is possible because the cue phrases ``\textit{had a dinner at}'' and ``\textit{where the food}'' both suggest there should be a restaurant entity between them.
We call such rationale phrases \textit{entity triggers} (or just {triggers}).

Prior works on trigger-aware NER primarily use a limited number of crowd-sourced triggers.
Although such triggers are of high quality, the crowd-sourcing procedure can be very expensive and time-consuming, as annotators are asked to provide both entity labels and their associated triggers in specifically designed annotation frameworks such as LEAN-LIFE~\cite{lee-etal-2020-lean}.
This largely limits the scale and domains of the collected entity triggers. 
In addition, these trigger-aware NER models (e.g., Trigger Matching Networks~\cite{lin-etal-2020-triggerner}) are built on  conventional sequence tagging architectures, e.g., BLSTM-CRFs~\cite{Lample2016NeuralAF}.
Few works connect entity triggers with contextualized embeddings from pre-trained language models such as BERT~\cite{Devlin2019BERTPO}, which can be highly beneficial for low-resource languages.
In this paper, we propose a novel two-stage NER framework, named \autotrigger, that can \textit{automatically} generate and exploit entity triggers with  pre-trained language models towards better generalization.

The \textit{first} stage of our framework (Sec.~\ref{ssec:soc}) aims to \textit{automatically extract entity triggers} using saliency map techniques based on input perturbations. 
Most saliency map techniques primarily focus on modeling the relative importance of each input token based on its 1) attention intensity~\cite{}, 2) gradients~\cite{} or 3) the changes of the output by excluding it from the input~\cite{}.
These methods can indeed produce useful explanations for some sentence classification tasks such as sentiment analysis, however, they are not well-aligned to our desired entity triggers --- a (potentially discontinuous) group of input tokens that often poses structural constraints to a target entity.
% \billquestion{can we have an example here?}
To address this challenge, we exploit the syntactic signals of sentences for properly assigning importance scores to a group of input tokens such that we can extract useful entity triggers without human efforts.
\textbf{[[LIZ: I don't totally understand what this has to do with syntactic signals of sentences? Just because you use parse constituents rather than randomly selected spans, or is there more to it?]]}

Specifically, 
for a given sentence and a target entity in it,
we first extract phrases from its \textit{constituency parsing tree}~\cite{} to form a collection of trigger candidates. 
Then, we score each trigger candidate by
testing its ability to predict the target entity in a variety of sampled contexts.
Here, we compare the system's ability to identify the target entity in versions of the sentence with and without the candidate trigger; if a trigger is indeed a meaningful clue for the model, then removing it should cause a noticeable drop in score. This \textit{sampling-and-occlusion} method is able to successfully identify high-quality triggers in a broad variety of domains. 
\textbf{[[LIZ: I agree with Bill, an example here would be good.]}
% computing the \textit{average score differences} between the input \textit{with} and \textit{without} the phrase in different context around the target candidate.
\billquestion{Add a concrete example? or reusing the one in the 2nd paragraph. }

The \textit{second} stage  (Sec.~\ref{ssec:tin})
focuses on how to use the extracted triggers for better performance and generalization of NER.
We propose \textit{Trigger Interpolation Network} (TIN), a novel architecture that effectively uses trigger-labeled NER data to train a model.
Since triggers are the most important non-entity words in an input sentence,
we want to strengthen our model's knowledge of these triggers. However, in many training instances, the entity words themselves are sufficient to learn an entity type, diluting the model's need to understand the surrounding context (including any triggers). To force the model to learn both words typically involved in entities as well as these ``most important'' trigger phrases, we employ two separate masking passes when learning our model's embeddings, one masking the entity words (forcing the model to rely more on the triggers) and one masking the triggers (forcing the model to rely more on the entity words). We then interpolate the embeddings of both entity-masked and trigger-masked sentences as the input to learn a mixed sentence representation as the input to standard sequence labeling.
In this manner, the TIN can effectively learn to exploit the triggers to infer entity boundaries and types with the powerful contextualized embeddings from pre-trained language models such as BERT.
% We leverages both entity triggers and pre-trained language model (BERT~\cite{}) into the NER task.
% We propose a novel model architecture that interpolates an entity masked sentence and trigger masked sentence.
% The underlying intuition of our proposed model is as follows:
% 1) For entity masked sentence, can the entity trigger itself determine the masked entity label?
% 2) For entity trigger masked sentence, how does the entity label prediction change when the entity triggers are masked?
% By interpolating the embedding outputs of both sentences, we could effectively model the relationship between entity and entity trigger.

Extensive experimental results on various domains of NER dataset show that our framework consistently outperforms baseline methods.
~\textcolor{red}{TODO: Mention human in the loop}

==> sections/sec_4_soc_sheikh.tex <==
\subsection{Automatic Trigger Extraction}
\label{ssec:soc}

In this first stage of our \textsc{AutoTriggER} framework, we adopt the \textit{sampling and occlusion} (\texttt{SOC}) algorithm for entity trigger extraction. \citet{jin2020towards} proposed SOC to analyze input for model interpretation. We adopt SOC, because it involves analysis of input at phrase-level for model prediction in contrast to the previous works~\citep{Ribeiro2016WhySI, li2016understanding} that focus on word-level analysis. SOC has been successfully employed to find important phrases that influence predictions from sequence classification models~\cite{}, but we adopt it for sequence tagging. 

Given an input instance of the labeled corpus $(\mathbf{x_i},\mathbf{y_i})\in\mathcal{D}_{L}$, we consider four primary steps to generate entity triggers: 1) phrase candidate $\mathcal{P}$, 2) entity token classifier $\mathcal{M}_t$, 3) phrase scoring, and 4) phrase selection.

\smallskip
\noindent
\textbf{Phrase Candidate.}\quad  

Given a training sentence, we construct a constituency parse tree from it and consider the set of phrase nodes, $\mathcal{P}$, from the tree as auto trigger candidates. Figure.~\ref{fig:soc} shows auto trigger candidates generated from constituency parsing of a sentence. The target entity mention (in this example  ``\textit{Cary Moon}'') is not included as a candidate. 

Note that the original \texttt{SOC} computes the word-level scores and extends to phrases by agglomerative clustering. Since clustering creates a large number of combinations of words to construct phrases, output phrases can be incomplete and noisy. By limiting the search space to a set of complete phrases, we could avoid such noisy triggers.

Mathematically, given an input instance $(\mathbf{x_i},\mathbf{y_i})\in\mathcal{D}_{L}$ and a target entity $e\in\mathbf{x_i}$, we generate a set of phrase candidate $\mathcal{P}=\{\mathbf{p_i}\}$ where $\mathbf{p_i} = (w_s,w_e)$ and $(w_s,w_e)$ is denoting the start and end index of the phrase span $\mathbf{p_i}$. To generate $\mathcal{P}$, we parse the input sentence $\mathbf{x_i}$ using constituency parsing and collect $\mathbf{p_i}$ corresponding to phrase nodes of the constituency-based parse tree. 
To avoid considering target entity as part of an entity trigger, we discard a set of entity-overlapped phrases $\{\mathbf{p_j}|e\in\mathbf{p_j}\}$.


\smallskip
\noindent
\textbf{Entity Token Classifier.}\quad 
The entity token classifier, $\mathcal{M}_t$, neural network that assigns a class label from a label set to a token in a sequence. Given an input sentence $\mathbf{x_i} = [x^{(1)}_i, x^{(2)}_i, \dots x^{(n)}_i]$, $\mathcal{M}_t$ classifies each token $x^{(j)}_i$ to the named entity tag $y^{(j)}_i \in \mathcal{Y}$ where $\mathcal{Y}$ is a predefined set of named entity tags such as B-PER, I-PER and O. Once we train $\mathcal{M}_t$ labeled corpus $\mathcal{D}_{L}$, we use it to derive a function $s$ that scores the target entity $e$ in the input sentence $\mathbf{x_i}\in\mathcal{D}_{L}$. Let the conditional probability $\mathbb{P}(\mathbf{y}|\mathbf{x})$ denote the output of $\mathcal{M}_t$. Then, $s$ computes the score of the target entity $e$ in $\mathbf{x}$ as the average conditional probability over tokens of the target entity $e$ using the following equation:
\begin{equation}
    \label{eq:seq_score}
    s(\mathbf{x}, e) = \frac{1}{|e|}\sum_{x^{(j)}\in e} \mathbb{P}(\mathbf{y^{(j)}}|x^{(j)}).
\end{equation}


\noindent
\textbf{Phrase Scoring.}\quad 
We use the phrase candidates set $\mathcal{P}$ and prediction score function $s$ derived from $\mathcal{M}_t$ to measure the importance score of each phrase $\mathbf{p} \in P$ towards target entity $e$ by sampling and occlusion (\texttt{SOC}) algorithm.
\texttt{SOC} is composed of two core methods: (1) \textit{input occlusion}, (2) \textit{context sampling}.
\begin{figure}[t]
    \centering 
    \includegraphics[scale=0.31]{figures/soc.pdf}
    \caption{\textbf{Overview of the Sampling and Occlusion (\textsc{SOC})}. It creates a set of phrase candidates with phrase nodes of the constituency parse tree, and then compute the phrase importance by average prediction difference between context sampled sentences and its phrase-masked sentences.
    % \billquestion{Can we enlarge the font size? Especially the part of ``Constituency Parse Tree''}
    }
    \label{fig:soc}
\end{figure}

\textit{Input occlusion}~\citep{li2016understanding} computes the importance of $\mathbf{p}$ specific to the entity $e$ in the input $\mathbf{x}$ by measuring the prediction difference caused by replacing the phrase $\mathbf{p}$ with padding tokens $0_\mathbf{p}$:
\begin{equation}
    \label{eq:importance}
    \phi(\mathbf{p}, \mathbf{x}, e)=s(\mathbf{x},e)-s\left(\mathbf{x}_{-\mathbf{p}}, e ; \mathbf{0}_{\mathbf{p}}\right).
\end{equation}
For example, in Figure.~\ref{fig:soc}, ``\textit{the next mayor}'' is replaced by pad tokens to compute its importance towards the entity ``\textit{Cary Moon}''.

However, the importance score $\phi(\mathbf{p}, \mathbf{x}, e)$ from equation~\ref{eq:importance} has a drawback that the $\mathbf{p}$ is dependent on context words around $\mathbf{p}$. It may neglect the fact that the importance score of $\mathbf{p}$ can vary depending on which context words are around the $\mathbf{p}$.

To eliminate the dependence, \textit{context sampling} samples the context words around the phrase $p$ and computes the average prediction differences over the samples. Specifically, it samples the context words $\hat{x}_{\delta}$ from a trained language model $p(\hat{x}_{\delta}|x_{-\delta})$ and obtains a set of context word replacements $\mathcal{S}$. For each replacement $\hat{x}_{\delta}\in\mathcal{S}$, we measure the prediction difference caused by replacing the phrase $\mathbf{p}$ with padding tokens. We take the average of these prediction differences to be the context-independent score $\phi(\mathbf{p}, \mathbf{x}, e)$ of the phrase $\mathbf{p}$, as expressed in equation \ref{eq:soc}:
\begin{equation} \label{eq:soc}
\resizebox{0.8\hsize}{!}{
\begin{split}
        \frac{1}{|\mathcal{S}|} \sum_{\hat{\mathbf{x}}_{\delta} \in \mathcal{S}}\left[s\left(\mathbf{x}_{-\delta},e ; \hat{\mathbf{x}}_{\delta}\right) - s\left(\mathbf{x}_{-\{\delta, \mathbf{p}\}},e ; \hat{\mathbf{x}}_{\delta} ; \mathbf{0}_{\mathbf{p}}\right)\right]
\end{split}
}
\end{equation}
In Figure.~\ref{fig:soc}, context words ``\textit{won't be}'' and ``\textit{of Seattle}'' around the phrase ``\textit{the next mayor}'' are replaced into ``\textit{will be}'' and ``\textit{of LA}'' which are sampled from the language model.
Then, the classifier computes the prediction difference between the sampled sentences with and without the phrase.

\smallskip
\noindent
\textbf{Phrase Selection.}\quad 
After obtaining the importance score $\phi(\mathbf{p}, \mathbf{x}, e)$ for all phrase candidates $\mathcal{P}=\{\mathbf{p_i}\}$,
we select the top $k$ candidate phrases with the highest importance score as the entity triggers, where $k$ is a hyperparameter. 
Specifically, for each input instance $(\mathbf{x_i},\mathbf{y_i})\in\mathcal{D}_{L}$, we pick the top $k$ candidate phrases as entity triggers $T(\mathbf{x_i},\mathbf{y_i})$ to create a form $\{(\mathbf{x_i}, \mathbf{y_i}, T(\mathbf{x_i},\mathbf{y_i}))\}$.



==> sections/sec_6_hitl.tex <==
\section{Human-in-the-Loop (HITL)} 
\label{ssec:hitl}

% As we mentioned, \textsc{SOC} in \textsc{AutoTriggER} trains the entity token classifier $\mathcal{M}_t$ with a labeled corpus $\mathcal{D}_L$, and derives a score function $s$ from trained $\mathcal{M}_t$.

We assume that training with automatically generated explanations or auto-triggers enables our model to look at tokens in a sentence that help to predict the label of an entity. 
Even though, by construction, a transformer model should achieve this through it's self-attention mechanism \citep{Devlin2019BERTPO}, it does not seem to learn this in a limited data scenario. 
Thus, larger performance gain from our model is observed in the limited data setting compared to other baseline transformers that do not take any help from auto-triggers. 

At training time, auto-triggers provide a form of weak supervision to help the model identify the tokens it should focus on. This is consistent with the finding of \citep{lee-etal-2020-lean, lin-etal-2020-triggerner}, where they use human selected triggers to provide this additional form of supervision. 
We observe a similar gain with auto-triggers without any human feedback. However, based on our findings we do conclude that we can leave humans out of the training process.
Rather, we propose to use the auto-triggers to further optimize the trigger annotation process for humans. We propose to skip the costly trigger highlighting process and refine a ranked list of auto-triggers using binary judgments from human. 

%In the inference stage, we do not need any trigger information. 
%Our model has the capacity to use explanations in the training phase and we hypothesize that at the inference stage it is able to  

%We leverage auto-triggers in a Human-in-the-loop (HITL) process to further improve model performance with optimal annotation effort. 

Our model, \autotrigger, has a hyperparameter which is the number of auto-triggers, and it is tuned using a validation set. 
According to our experiments, selecting the top-2, top-4, top-3, top-5 auto-triggers results in the best performance in the \conll, \bcdr, \laptop, and \wlp, respectively. 
However, we assume that this hard cut-off may result in less precision and recall in auto-trigger selection process.  
We assume that the performance can be further improved, if instead of considering only top-k auto-triggers, we take help from a human who provides binary judgments on a ranked list of auto-triggers found using SOC algorithm. We refer to these triggers as refined-auto-triggers. Based on human-centered computing literature \sheikh{CITE}, the filtering approach is cheaper compared to the selection approach, as spans are not required to be marked in a sentence. We still need to to show a fixed number of triggers to a human, but we can safely assume that this will result in both higher precision as well as recall -- making the trigger-based supervision more effective. 

We conduct a small-scale experiment with this approach and refine the trigger list found by the SOC algorithm in the CoNLL dataset. We show 10 ranked triggers to humans in our HITL phase, obtain refined-auto-triggers and train our model. A full-scale human annotation experiment is necessary to conclude the efficiency of such a new annotation process and compare it with existing trigger-annotation interfaces, such as the one provided by \citep{lee-etal-2020-lean}, we leave it as a future work.  


%In our previous experiments, we have found that even if triggers directly provided by humans are interpretable, they do not result in optimal performance, surpassing auto-triggers. That's why we leverage human assistance in filtering auto-triggers rather than selecting triggers from the sentences. Based on human-centered computing literature, the filtering approach is cheaper compared to the selection approach, as spans are not required to be marked in a sentence. Thus, with the help of humans, we can further increase the precision as well as recall of the auto-trigger selection process.   

% We have the following research questions but make assumptions for some of them for the sake of avoiding complicated evaluation: 
% \begin{itemize}
%     \item How to combine entity annotation and trigger annotation?
%     \item What is the size of the ranked list of triggers to be presented to human? 
%     \item When to take feedback for auto-triggers?
%     \item Is combining trigger annotation with entity annotation helpful? For example, we have a model trained on a limited amount of data. We take the model to an out-of-domain dataset. Now, we have some annotation budget. Should we only leverage that budget for entity annotation, or it is also useful to obtain annotation for auto-triggers. This mimics an active learning strategy. But, we will not retrain the model after a few round of annotation, rather we will do it in one shot. 
%     \item If our annotation budget is $k$ we have the following associated costs: 1. $C_{sentence}$: Cost of reading a sentence (The number of tokens in that sentence). 2. $C_{entity}$: Cost of judging the label for a selected entity (the number of tokens in the entity surface form). 3. $C_{trigger}$: Cost of judging the auto-trigger (the number of tokens in the trigger). 
%     \item We do a simple experiment, where we vary the number of sentences read by a human (as it is the costliest part of annotation), and the model performance with auto-triggers, and refined-auto-triggers. 
% \end{itemize}
% }
% \begin{figure}
%     \centering 
%     \includegraphics[scale=0.4]{figures/hitl.png}
%     \caption{HITL Proposal}
%     \label{fig:my_label}
% \end{figure}

==> sections/sec_9_ablation.tex <==
\subsection{Performance Analysis}

\smallskip
\noindent
\textbf{Trigger Candidate Variants.}
% \label{sec:trig_var}
In Sec~\ref{ssec:soc}, we first constructed a set of phrase candidates $\mathcal{P}$ for which the importance score is computed.
To show the efficacy of constituency parsing for constructing trigger candidates, we conduct an ablation study on different variants of it.
For the construction, we compare three variants:
(1) \texttt{RS} is random selection. It randomly chooses $n$ contiguous tokens to be grouped as a phrase for $k$ times.
Consequently, $\mathcal{P}$ is composed of $k$ random spans.
(2) \texttt{DP} is dependency parsing. Here, to generate $\mathcal{P}$, we first parse the input sentence using dependency parsing. Then, we traverse from the position of entity mention in the input sentence using depth-first-traversal and get a list of tokens visited for each hop up to 2-hops. Finally, for each hop, we convert the list of tokens to a list of phrases by merging the tokens that are contiguous into a single phrase. 
(3) \texttt{CP} is constituency parsing, which is our current method (see Sec.~\ref{ssec:soc}).
We expect each variant to provide different syntactic signals to our framework.
Figure~\ref{fig:triggervariants} shows the model's performance with triggers that have been selected from different sets of phrase candidates.
As we can see, constituency parsing yields consistently better performance by providing better quality of syntactic signals than others.

\begin{figure}[t]
\vspace{0.1cm}
\begin{minipage}{0.23\textwidth}
  \centerline{\includegraphics[width=4.6cm]{figures/conllbar.pdf}}
  \vspace{-0.1cm}
  \centerline{\small (a) CoNLL03}
\end{minipage}
\begin{minipage}{0.23\textwidth}
  \centerline{\includegraphics[width=4.6cm]{figures/bc5cdrbar.pdf}}
  \vspace{-0.1cm}
  \centerline{\small (b) BC5CDR}
\end{minipage}
\caption{Performance comparison (F1-score) of entity+trigger baselines on 20\% training dataset of CoNLL03 and BC5CDR with different trigger candidate variants.}
\label{fig:triggervariants}
\vspace{-0.2cm}
\end{figure}

\smallskip
\noindent
\textbf{Sensitivity Analysis of interpolation hyper-parameter ($\lambda$).}
In Sec~\ref{ssec:tin}, we linearly interpolated two different sources of knowledge by weight $\lambda$ 0.5.
To show how the weight $\lambda$ affects the performance, we conduct an ablation study on different $\lambda$ distribution.
As we can see from Figure.~\ref{fig:interpolation}, the framework achieves the highest performance when $\lambda$ is set to 0.5. It supports that the model achieves the best when we interpolate the entity and trigger knowledge in equal.

\begin{figure}[t]
\vspace{-0.1cm}
\begin{minipage}{0.23\textwidth}
  \centerline{\includegraphics[width=4.6cm]{figures/lambdabert.pdf}}
  \vspace{-0.1cm}
  \centerline{\small (a) BERT-TIN}
\end{minipage}
\begin{minipage}{0.23\textwidth}
  \centerline{\includegraphics[width=4.6cm]{figures/lambdaroberta.pdf}}
  \vspace{-0.1cm}
  \centerline{\small (b) RoBERTa-TIN}
\end{minipage}
\caption{Performance comparison (F1-score) of entity+trigger baselines on 20\% training dataset of BC5CDR with different interpolation weight $\lambda$.}
\vspace{-0.3cm}
\label{fig:interpolation}
\vspace{-0.0cm}
\end{figure}


==> sections/sec_a_related.tex <==
% \clearpage
\section{Related Work}
\label{sec:relatedwork}

% \smallskip
% \noindent
% \textbf{NER with Language Models.}\quad 

\smallskip
\noindent
\textbf{NER with Additional Supervision}
Previous and recent research has shown that encoding syntactic information into NER models compensate for the lack of labeled data \citep{syntactic_Tian2020ImprovingBN}. The improvement is consistent across word embedding based encoding (e.g. biLSTM) as well as unsupervised language model based encoding (e.g. BioBERT) of the given text. Typically, the external information that is encoded include POS labels, syntactic constituents, and dependency relations \citep{ syntactic_nie-etal-2020-improving, syntactic_Tian2020ImprovingBN}. The general mechanism to include linguistic information into NER model is to represent them using word vectors and then concatenate those representations with the original text representation. This approach fails to identify the importance of different types of syntactic information. Recently, \citet{syntactic_Tian2020ImprovingBN} and \citet{syntactic_nie-etal-2020-improving} both showed that key-value memory network (KVMN)  \citep{kvmn_miller2016key} are effective in capturing importance of linguistic information arising from different sources. KVMN has been shown to be effective in leveraging extra information, such as knowledge base entities, to improve question answering tasks. Before applying KVMN, contextual information about a token is encoded as the key and syntactic information are encoded as values. Finally, weights over the values are computed using the keys to obtain a representation of the values and concatenate it with the context features. Our approach uses token level features extracted by an explanation generation model, but later train to be able to pick-up those explanations directly from the text at inference time. 


%While this approach and other existing approaches model external knowledge, we use a model to identify tokens in a sentence that are useful for predicting entity type   


\smallskip
\noindent
\textbf{Limited Training Data for NER.}\quad 
The simplest way to approach the problem of limited data for NER is to use dictionary based weak supervision. An entity dictionary is used to retrieves unlabeled sentences from a corpus and weakly label them to create additional noisy data. This approach suffers from low recall as the training data covers a limited number of entities. The models tend to bias towards the surface form of the entities it has observed in the dictionary. There has also been approaches to retrieve sentences from a large corpus that are similar to sentences in the low-resource corpus to enrich it. These self-training approaches have been shown to be effective both in extremely limited data \citep{foley2018named, sarwar2018term} as well as limited data scenario \citep{du2020self}. Even though these data enhancement approaches explore a corpus to find related data cases, they do not exploit the explanation-based signals that is available within the limited data. 



\smallskip
\noindent
\textbf{Learning from Explanations.}\quad 
Recent works on Explainable AI are primarily focused on debugging the black box models by probing internal representations~\citep{ Adi2017FinegrainedAO, Conneau2018WhatYC},  testing model behavior using challenge sets~\citep{McCoy2019RightFT, Gardner2020EvaluatingML, Ribeiro2020BeyondAB}, or analyzing an impact of input examples by input perturbations or influence function looking at input examples~\citep{Ribeiro2016WhySI, Koh2017UnderstandingBP}. However, for an explanation of the model to be effective, it must provide not only the reasons for the model's prediction but also suggestions for corresponding actions in order to achieve an objective. 
% To address the limitation, prior works have studied regularizing the neural networks by model’s explanation \citep{Ross2017RightFT, Plumb2020RegularizingBM}. Even so, if the model explanations do not match human judgment or domain expertise, those models may not be trained as we expect.
Efforts to cope with this issue by incorporating human explanations into the model are called Explanation-based learning~\citep{DeJong2004ExplanationbasedLA}. 
These works are aiming to exploit generalized explanations for drawing inferences from unlabeled data while maintaining model transparency. Most prior works on explanation-based learning are mainly focused on facilitating logical rules as an explanation. They use such rules to create weak supervision~\citep{Ratner2017SnorkelRT} and regularize posterior~\citep{Hu2016HarnessingDN, Hu2017TowardCG}. Another form of explanations can be specific words in the sentence which aligns to our work. Notable work in this line asks annotators to highlight important words, then learn a generative model over parameters given these rationales~\citep{Zaidan2008ModelingAA}.

% Taking advantage of the natural language’s infinite space of reasoning and expression, recent works attempt to incorporate the natural language form of explanation into the model. Attempts are made by exploiting language to directly produce model parameters \citep{Ba2015PredictingDZ}, as part of the parameter space \citep{Andreas2018LearningWL}, and to train models that generate their own explanations \citep{Camburu2018eSNLINL, Rajani2019ExplainYL}. While the above works view language from an instance-level explanation perspective, recent works explore global-level explanation. They use semantic parsers to convert language into a global collection of features and noisy labels on unlabeled data via hard matching \citep{Srivastava2017JointCL, Hancock2018TrainingCW}. However, recent works on global-level natural language explanation have two main drawbacks: 1) neglecting the importance of linguistic variants, thus resulting in a very low recall. 2) predictions of oversimplified labeling function are overly confident. These drawbacks are the result of limiting the infinite space of reasoning and expression in natural language.

% Our proposal is mainly focused on maximizing the generalization ability of natural language explanations by making the most of the infinite expressive power of natural language. To make this possible, we are proposing a soft matching module that can be utilized not only in IE tasks but also in general NLP applications further. By enabling fully leveraging natural language form of explanation, we expect three far-reaching implications: 1) The format of the labeling function is not restricted, making it easy to collect, and furthermore, it could be retrieved from the text corpus. 2) If the answer is wrong, the user may be able to directly teach the system by providing explanations. 3) Unlike the recent trend of explainable AI, which analyzes input examples, we can analyze how explanations affect the model predictions.

